Understanding the Impact of Edge Cases from Occluded Pedestrians for ML Systems

Machine learning (ML)-enabled approaches are considered a substantial support technique of detection and classification of obstacles of traffic participants in self-driving vehicles. Major breakthroughs have been demonstrated the past few years, even covering complete end-to-end data processing chain from sensory inputs through perception and planning to vehicle control of acceleration, breaking and steering. YOLO (you-only-look-once) is a state-of-the-art perception neural network (NN) architecture providing object detection and classification through bounding box estimations on camera images. As the NN is trained on well annotated images, in this paper we study the variations of confidence levels from the NN when tested on hand-crafted occlusion added to a test set. We compare regular pedestrian detection to upper and lower body detection. Our findings show that the two NN using only partial information perform similarly well like the NN for the full body when the full body NN's performance is 0.75 or better. Furthermore and as expected, the network, which is only trained on the lower half body is least prone to disturbances from occlusions of the upper half and vice versa.

==> backup.tex <==
\newpage
\section{Notes:}
Target: SEAA 2021. Deadline 1 April 2021
\newpage
\section{Introduction}
The purpose of this paper is to identify a niche that can be followed through the remaining two years of the phd. Target is IVS 2021, deadline 15th Feb.

\subsection{What}
The target topic is evaluation of safety properties such as how to handle outliers or scenarios outside of the scope of the model. To evaluate safety we might need functional descriptions of ML, that is to be covered by Software engineering fields. 

The topic may or may not include 
\begin{itemize}
    \item Utilizing history in deep nets (LSTM/ Feedback systems, physical laws etc.) 
    \item V\&V protocol for DNN
    \item Specific measures (instruments) that highlight sufficiency's / insufficiencies in the DNN
\end{itemize}

\subsection{How?}
Through reference snowballing on ACM and IEEE online libraries. arxiv: We can use this to get pre-prints and more open access papers. 

\begin{itemize}
    \item Start with going through the ~100 citations of ODIN from NASA-ADS (Reference from ARXIV). Extract those citations into endnote and study its content.
    \item Determine based on abstract if a paper is relevant towards: a) Prediction robustness/reliability/uncertainty. b) Safety/Decision explainability/autonomous driving. c) out-of-distribution samples. 
    \item read included papers 
\end{itemize}



\subsection{Starting point}
Waymo recently published their findings for ADS: 
\href{https://waymo.com/safety/}{Waymo Safety}. It contains a few set of references that can be used. No citations found so far (See question below). 

Way of working: Logic for Design Science Research Theory Accumulation. Mainly to catch changes in dataset or scope of the model. 

Enhancing the robustness of out-of-distribution networks. 

The ESPLENADE paper 


\subsection{Inclusion criteria}
\textbf{Q: Do we limit ourselves based on which sensor they test on}? \textit{A: Depends on the size of papers found. Exclude everything except cameras if we have a large portion of data. }
\begin{itemize}
    \item \textbf{"Supervisor"}: Covers a method that highlights performance of the model, when encountering outliers. 
    \item \textbf{SWE Aspects:} Covers safety/integrity/robustness aspects of deep learning.
    \item \textbf{ADS Safety}: Covers Safety or deployment of ADS including ML. 
    \item Methods for explainability in machine learning. "Why" is a model misbehaving. 
    \item Pre-cond. for explainability: how is the network reasoning, i.e through studying feature maps, how does certain inputs map to certain features. Are there any connection here? 
\end{itemize}

\subsection{Questions}
\begin{itemize}
    \item \textbf{Q: How to prove safety without full coverage? How is coverage defined for a deep neural net?} -- \textit{A: It is simpler to prove that a system is unsafe, and build your argumentation from that p.o.v instead. }
    \item \textbf{What is the operative architecture like? Does this affect the instruments that ensure credibility of the network?} -- \textit{We can limit ourselves to the subcomponent "Deep learning", otherwise it would be too complex. }
    \item \textbf{How to cite non-published material like the Waymo report? The report covers testing on larger scale compared to published materials. Likewise, it has no references.} -- \textit{A:  Consider it a white paper/Wikipedia page from Waymo. Save a copy and date of the paper when accessed, and then it is OK to cite.}   
\end{itemize}


1 Look at a different dataset / Model
2 Add an extra OOD method? 
3a How much effort to compare all of the methods.
3b Look at a sequence of frames?


- First step would be to use SEAA setup, but on Waymo data. What would then be the outlier dataset? 
    - A trained model on Waymo? 
    - Download an outlier set? 
    - Adapt the OOD methods? 
    - What can Stig and Christian help with? 
